Prompt Recovery for Image Generation Models: A Comparative Study of Discrete Optimizers

Recovering natural language prompts for image generation models, solely based on the generated images is a difficult discrete optimization problem. In this work, we present the first head-to-head comparison of recent discrete optimization techniques for the problem of prompt inversion. We evaluate Greedy Coordinate Gradients (GCG), PEZ , Random Search, AutoDAN and BLIP2's image captioner across various evaluation metrics related to the quality of inverted prompts and the quality of the images generated by the inverted prompts. We find that focusing on the CLIP similarity between the inverted prompts and the ground truth image acts as a poor proxy for the similarity between ground truth image and the image generated by the inverted prompts. While the discrete optimizers effectively minimize their objectives, simply using responses from a well-trained captioner often leads to generated images that more closely resemble those produced by the original prompts.

==> figures/name.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{.66\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{figures/quantitative_results/images/CLIP_SCORE_INV_PROMPT_TO_BASE_IMAGE.pdf}
      \caption{Original images v. recovered images}
      \label{fig:quant:fid}
    \end{subfigure}%
    ~
    \begin{subfigure}{.34\textwidth}
      \centering
      \includegraphics[height=0.99\linewidth]{figures/quantitative_results/images/intermediate_CLIP_SCORE_INV_PROMPT_TO_BASE_IMAGE.pdf}
      \caption{Change During Optimization}
      \label{fig:quant:clip_base_to_inv}
    \end{subfigure}
    
    \caption{to add} 
    \label{fig:quant}
\end{figure}

==> figures/qualitative_results/example_2/table.tex <==

    \noindent\fbox{%
        \parbox{\textwidth}{%
            \begin{tabular}{@{} m{0.28\textwidth} m{0.67\textwidth} @{}}
                % Adjust vertical alignment of the image and table to the top
                \adjustbox{valign=t}{\includegraphics[width=\linewidth,keepaspectratio]{figures/qualitative_results/example_2/example.png}} 
                &
                % Minipage for the internal table to keep it aligned
                \begin{minipage}[t]{\linewidth}
                    % Adjust array stretch for row height and row colors for alternate shading
                    \renewcommand{\arraystretch}{1.5} % Reduce vertical space between rows
                    \rowcolors{1}{gray!15}{white} 
                    % Internal table with better label formatting and readable captions
                    \begin{tabular}{>{\raggedright\arraybackslash}m{0.2\linewidth}|>{\raggedright\arraybackslash}m{0.75\linewidth}} 
                        \textbf{\footnotesize{Original Prompt}} &  \footnotesize{concept art of giant translucent glowing jellyfishes, renaissance, divers helmet, lots of teeth, melting horror, round moon, rich clouds, fighting the horrors of the unknown, mirrors, very detailed, volumetric light, mist, grim, fine art, decaying, textured oil over canvas, epic fantasy art, very colorful, ornate, anato finnstark } \\
                        \hline
                        \textbf{\footnotesize{PRISM}} &  \footnotesize{Vibrant surreal jellyfish scene above calm water, orange and red tops with textures, colorful whimsical sky, round object floating above.} \\
                        \hline
                        \textbf{\footnotesize{BLIP-2}} &  \footnotesize{jellyfish floating in the ocean with many other jellyfish floating around it in the sky above it with the moon in the background and the sun in the middle of} \\
                        \hline
                        \textbf{\footnotesize{AutoDAN w/ Prior}} &  \footnotesize{ mushroom colony floating west upon winds \| Image illustration show red colony eating jelly monster) \$} \\
                        \hline
                        \textbf{\footnotesize{AutoDAN w/o Prior}} & \footnotesize{scifi crablandscape utz retweeted science ffice winners fish red ) jelly pizzeria kimbun:\-) \(\*railways ___ standings}  \\
                        \hline
                        \textbf{\footnotesize{PEZ}} &  \footnotesize{fantasy magideviantart minemeatballs giantbeavs cannedemdebate residences amidst underwater tulips antarctica jellyfish........... ufo katrindeviantart sensual} \\
                        \hline
                        \textbf{\footnotesize{GCG}} & \footnotesize{movingpresser nightmare ho>:!\"\@ avg madddownloadable jeter visitspain mushroom red xoxhqalyssa ritz.\# marinelandscape}  \\
                        \hline
                        \textbf{\footnotesize{Random Search}} & \footnotesize{athing hse ate facezzzz waltopus seas \~hq warmly mushrooms cannemolecules plankton ). pieter thunderstorm redplains} \\
                    \end{tabular}
                \end{minipage}
            \end{tabular}
        }
    } 
    

==> figures/qualitative_results/example_3/table.tex <==

    \noindent\fbox{%
        \parbox{\textwidth}{%
            \begin{tabular}{@{} m{0.28\textwidth} m{0.67\textwidth} @{}}
                % Adjust vertical alignment of the image and table to the top
                \adjustbox{valign=t}{\includegraphics[width=\linewidth,keepaspectratio]{figures/qualitative_results/example_3/example.png}} 
                &
                % Minipage for the internal table to keep it aligned
                \begin{minipage}[t]{\linewidth}
                    % Adjust array stretch for row height and row colors for alternate shading
                    \renewcommand{\arraystretch}{1.5} % Reduce vertical space between rows
                    \rowcolors{1}{gray!15}{white} 
                    % Internal table with better label formatting and readable captions
                    \begin{tabular}{>{\raggedright\arraybackslash}m{0.2\linewidth}|>{\raggedright\arraybackslash}m{0.75\linewidth}} 
                        \textbf{\footnotesize{Original Prompt}} &  \footnotesize{cute baby chick dressed with inmate clothes } \\
                        \hline
                        \textbf{\footnotesize{PRISM}} &  \footnotesize{Baby in bright yellow outfit and hat, sitting on gray background, serious expression, shiny belt.} \\
                        \hline
                        \textbf{\footnotesize{BLIP-2}} &  \footnotesize{baby dressed in a yellow costume sitting on a gray background stock photo} \\
                        \hline
                        \textbf{\footnotesize{AutoDAN w/ Prior}} &  \footnotesize{little infant dressed \- photo: Creative Assembly Download mock top hats Mock gold pants Suit sweater Yellow \'74} \\
                        \hline
                        \textbf{\footnotesize{AutoDAN w/o Prior}} & \footnotesize{minions pediatric photograph photography delaney studios........... > matte horst top lamb sleeve shoes m j,!\' \[ \';}  \\
                        \hline
                        \textbf{\footnotesize{PEZ}} &  \footnotesize{comforting filet genius rabbit baby cosplay looked mustard courtesy jason goon regards aliaa ghtyphotog photograph yotpo quadcopter screenshotphotographer} \\
                        \hline
                        \textbf{\footnotesize{GCG}} & \footnotesize{ctugette ty souls wexmondays elmo lemon)/ chedrealistic cottonbaby beret pajamas photog chadsaul\"\- rockabsaura}  \\
                        \hline
                        \textbf{\footnotesize{Random Search}} & \footnotesize{. tten. floorinevcheesmango peakdistrict infant character \| bestofdeli campaign awawool uniforms mannyjamiedorqx} \\
                    \end{tabular}
                \end{minipage}
            \end{tabular}
        }
    } 
    

==> figures/qualitative_results/example_4/table.tex <==

    \noindent\fbox{%
        \parbox{\textwidth}{%
            \begin{tabular}{@{} m{0.28\textwidth} m{0.67\textwidth} @{}}
                % Adjust vertical alignment of the image and table to the top
                \adjustbox{valign=t}{\includegraphics[width=\linewidth,keepaspectratio]{figures/qualitative_results/example_4/example.png}} 
                &
                % Minipage for the internal table to keep it aligned
                \begin{minipage}[t]{\linewidth}
                    % Adjust array stretch for row height and row colors for alternate shading
                    \renewcommand{\arraystretch}{1.2} % Reduce vertical space between rows
                    \rowcolors{1}{gray!15}{white} 
                    % Internal table with better label formatting and readable captions
                    \begin{tabular}{>{\raggedright\arraybackslash}m{0.2\linewidth}|>{\raggedright\arraybackslash}m{0.75\linewidth}} 
                        \textbf{\footnotesize{Original Prompt}} &  \footnotesize{an army of space soldiers invading an ice world full of mountains and rocks, award winning, trending on artstation, unreal engine} \\
                        \hline
                        \textbf{\footnotesize{PRISM}} &  \footnotesize{seven metallic armored astronauts, holding weapons, icy rocky landscape, blue lighting, ready stance} \\
                        \hline
                        \textbf{\footnotesize{BLIP-2}} &  \footnotesize{group of soldiers standing in front of an ice cave with a blue light in the background, 3 d illustration} \\
                        \hline
                        \textbf{\footnotesize{AutoDAN w/ Prior}} &  \footnotesize{player entering ice armour formation beneath frost trolls shown standing along white tiger stripes during summer Time. Large background} \\
                        \hline
                        \textbf{\footnotesize{AutoDAN w/o Prior}} & \footnotesize{callister clones roaming glacier facing armour trademark during descent sands \-\- (pxbeanie jo trek league rudolph hgcsp}  \\
                        \hline
                        \textbf{\footnotesize{PEZ}} &  \footnotesize{scifi campaminiatures ssal troopparticipants featuring arctic kul centre freezing campasuit helmets appear depicting underwater ice cliffs environments} \\
                        \hline
                        \textbf{\footnotesize{GCG}} & \footnotesize{hrasverdun join drautodayinreborn mutant bj azugrontroopers youcanas glacial frost \# confedershervault}  \\
                        \hline
                        \textbf{\footnotesize{Random Search}} & \footnotesize{nevescifi rium ikonchafbergs testammarines arrillanarctic. blakemerrychristmas \` dlc kampgettable celticfc frigh} \\
                    \end{tabular}
                \end{minipage}
            \end{tabular}
        }
    } 
    

==> figures/quantitative_formatting.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{figures/quantitative_results/FID.pdf}
      \caption{Original images v. recovered images}
      \label{fig:quant:fid}
    \end{subfigure}%
    ~
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{figures/quantitative_results/CLIP_SCORE_BASE_PROMPT_TO_INV_IMAGE.pdf}
      \caption{Original prompts v. recovered images}
      \label{fig:quant:clip_base_to_inv}
    \end{subfigure}
    \\
    \vspace{12pt}
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{figures/quantitative_results/CLIP_SCORE_INV_PROMPT_TO_BASE_IMAGE.pdf}
      \caption{Original images v. recovered prompts}
      \label{fig:quant:clip_inv_to_base}
    \end{subfigure}%
    ~
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{figures/quantitative_results/TEXT_EMBEDDING_SIMILARITY.pdf}
      \caption{Original prompts v. recovered prompts}
      \label{fig:quant:cosine}
    \end{subfigure}
    
    \caption{Performance comparisons across four metrics:  (a) the FID between images generated by the original prompt and the inverted prompts; (b) the CLIP Score between the original prompt and the images generated by the inverted prompts; (c) CLIP Score between the inverted prompts and the images generated by the original prompt (Note that this is the optimization objective); (d) Cosine Similarity between CLIP text embeddings for the original and inverted prompts.} 
    \label{fig:quant}
    
\end{figure}

==> figures/quantitative_results/clip_score_base_prompt_to_inv_image.tex <==

\begin{subfigure}{.66\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth]{figures/quantitative_results/images/CLIP_SCORE_BASE_PROMPT_TO_INV_IMAGE}
  \label{fig:quant:CLIP_SCORE_BASE_PROMPT_TO_INV_IMAGE}
  \caption{CLIP Similarity}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[height=0.99\linewidth]{figures/quantitative_results/images/intermediate_CLIP_SCORE_BASE_PROMPT_TO_INV_IMAGE.pdf}
    \caption{Optimization Trajectories}
  \label{fig:quant:intermediate_CLIP_SCORE_BASE_PROMPT_TO_INV_IMAGE}
\end{subfigure}
            
